Real-Time Metric-Semantic Mapping for Autonomous Navigation in Outdoor Environments

The creation of a metric-semantic map, which encodes human-prior knowledge, represents a high-level abstraction of environments. However, constructing such a map poses challenges related to the fusion of multi-modal sensor data, the attainment of real-time mapping performance, and the preservation of structural and semantic information consistency. In this paper, we introduce an online metric-semantic mapping system that utilizes LiDAR-Visual-Inertial sensing to generate a global metric-semantic mesh map of large-scale outdoor environments. Leveraging GPU acceleration, our mapping process achieves exceptional speed, with frame processing taking less than 7ms, regardless of scenario scale. Furthermore, we seamlessly integrate the resultant map into a real-world navigation system, enabling metric-semantic-based terrain assessment and autonomous point-to-point navigation within a campus environment. Through extensive experiments conducted on both publicly available and self-collected datasets comprising 24 sequences, we demonstrate the effectiveness of our mapping and navigation methodologies. Code has been publicly released: https://github.com/gogojjh/cobra

==> chapter/biography.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.0in,clip,keepaspectratio]{figure/bio/jjh.png}}]{Jianhao Jiao}(Member, IEEE)
    received the B.Eng. degree in instrument science from Zhejiang University, Hangzhou, China, in 2017, and the Ph.D. from the Department of Electronic and Computer Engineering, the Hong Kong University of Science and Technology, Hong Kong, China.
    He is currently a senior research fellow with the Department of Computer Science, University College London.
    His research interests include navigation and embodied intelligence.
    % He is an Associate Editor of IEEE IROS 2024.
\end{IEEEbiography}
\vspace{-1.4cm}

\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.0in,clip,keepaspectratio]{figure/bio/ruoyu_geng_2}}]{Ruoyu Geng}
    received the B.S. degree from Jilin University, Changchun, China.
    She is currently a Ph.D student in Department of Robotics and Autonomous Systems, Hong Kong University of Science and Technology (Guangzhou). Her research interest mainly focuses on learning-aided SLAM and semantic segmentation.
\end{IEEEbiography}
\vspace{-1.4cm}

\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.0in,clip,keepaspectratio]{figure/bio/lyh}}]{Yuanhang Li}
    received the B.S. degree from Xiamen University, Xiamen, China in 2021.
    He has been a Ph.D. student in Department of Electronic and Computer Engineering, Hong Kong University of Science and Technology since 2022. His areas of research include Multi-Object Tracking and Trajectory Planning algorithms.
\end{IEEEbiography}
\vspace{-1.4cm}

\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.0in,clip,keepaspectratio]{figure/bio/renxin_color.png}}]{Ren Xin}
    received the B.Eng. degree in Mechanical Design and its Automation from Ocean University of China, Qingdao, China. He is currently a PhD student in Department of Robotics and Autonomous Systems, Hong Kong University of Science and Technology (Guangzhou). His research interest mainly focuses on learning based methods of path planning, motion prediction and map representations.
\end{IEEEbiography}
\vspace{-1.4cm}

\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.0in,clip,keepaspectratio]{figure/bio/bowen_color.png}}]{Bowen Yang}
    received the B.Eng. degree in the Hong Kong Polytechnic University, China, in 2019.
    He is currently pursuing the Ph.D. degree in the Department of Electronic and Computer Engineering, the Hong Kong University of Science and Technology, China.
    His research mainly focuses on scene understanding and path planning for autonomous robots.
\end{IEEEbiography}
\vspace{-1.4cm}

\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.0in,clip,keepaspectratio]{figure/bio/wujin_color}}]{Jin Wu}
    received the B.S. degree from University of Electronic Science and Technology of China, Chengdu, China.
    He has been a research assistant since 2018, and now a Ph.D. student in Department of Electronic and Computer Engineering, Hong Kong University of Science and Technology. He was with Tencent Robotics X, Shenzhen, China from 2019 to 2020. During 2012 to 2018, he was in the UAV industry and has brought up two companies.
\end{IEEEbiography}
\vspace{-1.4cm}

\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.0in,clip,keepaspectratio]{figure/bio/lujia_wang_color}}]{Lujia Wang}
    received the Ph.D. degree from the Department of Electronic Engineering, The Chinese University of Hong Kong, Sha Tin, Hong Kong, in 2015. From 2016 to 2021, she was an Associate Professor with the Shenzhen Institutes of Advanced Technology, Chinese Academy of Sciences, Shenzhen, Guangdong. She is currently a senior lecturer of the Red Bird MPhil program at the Hong Kong University of Science and Technology (Guangzhou).
\end{IEEEbiography}
\vspace{-1.4cm}

% \begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.0in,clip,keepaspectratio]{figure/bio/rfan.jpg}}]{Rui Fan}(Senior Member, IEEE)
%     received the B.Eng. degree in automation from the Harbin Institute of Technology in 2015 and the Ph.D. degree in electrical and electronic engineering from the University of Bristol in 2018. He worked as a Research Associate at the Hong Kong University of Science and Technology from 2018 to 2020 and a Postdoc Fellow at the University of California San Diego between 2020 and 2021.
%     He is currently a full Professor at Tongji University and Shanghai Research Institute for Intelligent Autonomous Systems.
%     % Rui was named in Stanford University List of Top 2\% Scientists Worldwide in 2022. His research interests include computer vision, deep learning, and robotics.
% \end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.0in,clip,keepaspectratio]{figure/bio/ming_color.png}}]{Ming Liu}(Senior Member, IEEE)
    % received the Ph.D. degree from the Department of Mechanical and Process Engineering, ETH Zurich, Switzerland, in 2013, supervised by Prof. Roland Siegwart.
    % During his master's study with Tongji University, he stayed one year with the Erlangen-Nunberg University and ¨Fraunhofer Institute IISB, Erlangen, Germany, as a Master Visiting Scholar. 
    % He is currently with the Robotics and Autonomous Systsms, The Hong Kong University of Science and Technology (Guangzhou), the director of Intelligent Autonomous Driving Center, as an Associate Professor.
    % He has published many popular papers in top journals including IEEE Transactions on Robotics and International Journal of Robotics Research. Dr. Liu is currently an Associate Editor for IEEE Robotics and Automation Letters, IET Cyber-Systems and Robotics, International Journal of Robotics and Automation.
    % He is also a founding member of Shanghai Swing Automation Ltd., Co. He is coordinating and involved in NSF Projects and National 863-Hi-TechPlan Projects in China. 
    % His research interests include dynamic environment modeling, deep-learning for robotics, 3D mapping, machine learning, and visual control.
    received the Ph.D. degree from the Department of Mechanical and Process Engineering, ETH Zurich, Zurich, Switzerland, in 2013, supervised by Prof. Roland Siegwart.
    He is currently an Associate Professor with Robotics and Autonomous Systems, Hong Kong University of Science and Technology (Guangzhou).
    % where he is also the Director of Intelligent Autonomous Driving Center, coordinating research and development on robotics and logistics.
    % His research works have been widely reported in over 300 journal and conference papers.
    % He was an Associate Editor of \textsc{IEEE Robotics and Automation Letters} and a committee member of RSS 2021.
    % Dr. Liu was a recipient of the European Micro Aerial Vehicle Competition (EMAV’09) (second place) and two awards from International Aerial Robot Competition (IARC’14) as a Team Member, the Best Student Paper Award as first author for MFI 2012 (IEEE International Conference on Multisensor Fusion and Information Integration), the Best Paper Award in Information for IEEE International Conference on Information and Automation (ICIA 2013) as first author, the Best Paper Award Finalists as co-author, the Best RoboCup Paper Award for IROS 2013 (IEEE/RSJ International Conference on Intelligent Robots and Systems), the Best Conference Paper Award for IEEE-CYBER 2015, the Best Student Paper Finalist for RCAR 2015 (IEEE International conference on Real-time Computing and Robotics), the Best Student Paper Finalist for ROBIO 2015, the Best Student Paper Award for IEEE-ICAR 2017, the Best Paper in Automation Award for IEEE-ICIA 2017, twice the innoviation contest Chunhui Cup Winning Award in 2012 and 2013, and the Wu Wenjun AI Award in 2016. He was the Program Chair of IEEERCAR 2016 and the Program Chair of International Robotics Conference in Foshan 2017. He was the Conference Chair of ICVS 2017.
    % He has published many popular papers in top journals including IEEE TRANSACTIONS ON ROBOTICS (TRO) and INTERNATIONAL JOURNAL OF ROBOTICS RESEARCH (IJRR). Dr. Liu is currently an Associate Editor for IEEE ROBOTICS AND AUTOMATION LETTERS, IET CYBER-SYSTEMS AND ROBOTICS, INTERNATIONAL JOURNAL OF ROBOTICS AND AUTOMATION. He is a Senior Member of IEEE.
\end{IEEEbiography}
\vspace{-1.4cm}

\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.0in,clip,keepaspectratio]{figure/bio/rfan.jpg}}]{Rui Fan}(Senior Member, IEEE) began his faculty career as a Full Research Professor with the College of Electronics \& Information Engineering at Tongji University in 2021, and was then promoted to a Full Professor in the same college, as well as at the Shanghai Research Institute for Intelligent Autonomous Systems in 2022. His research interests include computer vision, deep learning, and robotics, with a specific focus on humanoid visual perception under the two-streams hypothesis.
\end{IEEEbiography}
\vspace{-1.4cm}

\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.0in,clip,keepaspectratio]{figure/bio/kanoulas.png}}]{Dimitrios Kanoulas}
    received the Ph.D. degree from Northeastern University, Boston. He was a Postdoctoral Researcher at the Italian Institute of Technology for five years. He is currently a Professor of Robotics and AI with the Department of Computer Science, University College London (UCL), and a UKRI Future Leaders Fellow (FLF).
    % He worked on several real-world humanoid and animaloid robots.
    He has published more than 50 research papers in high-impact robotic journals and conferences.
    % His research interests include robot cognition, planning, and learning. 
    % He received the Best Interactive Paper Award from IEEE Humanoids 2017, the Best Student Paper Award Finalist from IEEE ICARCV 2018, the Outstanding Associate Editor Award from IEEE/RSJ IROS 2022, the U.K.-RAS Early Career Award 2022, and the Outstanding Paper Finalist at ICML (WFVML workshop) 2023.
\end{IEEEbiography}
\vspace{-1.4cm}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{ming2.png}}]{Ming Liu} received the B.A. degree in automation from Tongji University, Shanghai, China,
% in 2005, and the Ph.D. degree from the Department of Mechanical and Process Engineering, ETH Zurich, Zurich, Switzerland, in 2013, supervised by
% Prof. Roland Siegwart. During his master's study with Tongji University, he stayed one year with the Erlangen-Nunberg University and Fraunhofer Institute IISB, Erlangen, Germany, as a Master Visiting Scholar.\\
% \indent He is currently with the Electronic and Computer Engineering, Computer Science and Engineering Department, Robotics Institute, The Hong Kong University of Science and Technology (HKUST), Hong Kong, China, as an Associate Professor. He is also a founding member of Shanghai Swing Automation Ltd., Co. He is currently the chairman of Shenzhen Unity Drive Inc., China. He is coordinating and involved in NSF Projects and National 863-Hi-TechPlan Projects in China. His research interests include dynamic environment modelling, deep-learning for robotics, 3-D mapping, machine learning, and
% visual control.\\
% \indent Dr. Liu was a recipient of the European Micro Aerial Vehicle Competition
% (EMAV'09) (second place) and two awards from International Aerial Robot
% Competition (IARC'14) as a Team Member, the Best Student Paper Award
% as first author for MFI 2012 (IEEE International Conference on Multisensor
% Fusion and Information Integration), the Best Paper Award in Information
% for IEEE International Conference on Information and Automation (ICIA
% 2013) as first author, the Best Paper Award Finalists as co-author, the Best
% RoboCup Paper Award for IROS 2013 (IEEE/RSJ International Conference
% on Intelligent Robots and Systems), the Best Conference Paper Award for
% IEEE CYBER 2015, the Best Student Paper Finalist for RCAR 2015 (IEEE
% International conference on Real-time Computing and Robotics), the Best
% Student Paper Finalist for IEEE ROBIO 2015, the Best Student Paper for IEEE ROBIO 2019, the Best Student Paper Award for IEEE ICAR 2017, the Best Paper in Automation Award for IEEE ICIA 2017, twice the innoviation contest Chunhui Cup Winning Award in 2012 and 2013, and the Wu Wenjun AI Award in 2016. He was the Program Chair of IEEE RCAR 2016 and the Program Chair of International Robotics Conference in Foshan 2017. He was the Conference Chair of ICVS 2017. He has published many popular papers in top robotics journals including \textsc{IEEE Transactions on Robotics}, \emph{International Journal of Robotics Research} and \textsc{IEEE Robotics and Automation Magazine}. \\
% \indent Dr. Liu is currently an Associate Editor for \textsc{IEEE Robotics and Automation Letters}, \emph{International Journal of Robotics and Automation}, \emph{IET Cyber-Systems and Robotics}, IEEE IROS Conference 2018, 2019 and 2020. He was also an associate editor of special issue in \textsc{IEEE Transactions on Automation Science and Engineering}. He is a Senior Member of IEEE.

%Dr. Liu was a recipient of the European Micro Aerial Vehicle Competition
%(EMAV'09) (second place) and two awards from International Aerial Robot
%Competition (IARC'14) as a Team Member, the Best Student Paper Award
%as first author for MFI 2012 (IEEE International Conference on Multisensor
%Fusion and Information Integration), the Best Paper Award in Information
%for IEEE International Conference on Information and Automation (ICIA
%2013) as first author, the Best Paper Award Finalists as co-author, the Best
%RoboCup Paper Award for IROS 2013 (IEEE/RSJ International Conference
%on Intelligent Robots and Systems), the Best Conference Paper Award for
%IEEE CYBER 2015, the Best Student Paper Finalist for RCAR 2015 (IEEE
%International conference on Real-time Computing and Robotics), the Best
%Student Paper Finalist for IEEE ROBIO 2015, the Best Student Paper for IEEE ROBIO 2019, the Best Student Paper Award for IEEE ICAR 2017, the Best Paper in Automation Award for IEEE ICIA 2017, twice the innoviation contest Chunhui Cup Winning Award in 2012 and 2013, and the Wu Wenjun AI Award in 2016. He was the Program Chair of IEEE RCAR 2016 and the Program Chair of International Robotics Conference in Foshan 2017. He was the Conference Chair of ICVS 2017. He has published many popular papers in top robotics journals including \textsc{IEEE Transactions on Robotics}, \emph{International Journal of Robotics Research} and \textsc{IEEE Transactions on Automation Science and Engineering}. 
% \end{IEEEbiography}


==> chapter/exp_table_mapping_result_format_1.tex <==
\begin{comment}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[t]
  \centering
  \caption{mapping result}
  \renewcommand\arraystretch{1.2}
  \renewcommand\tabcolsep{11pt}
  \begin{tabular}{ccccccccccccc}
    \toprule
    \multirow{2}{*}{Dataset}                 & \multirow{2}{*}{Seq.}   & \multicolumn{3}{c}{\text{VoxField}} & \multicolumn{3}{c}{\text{Ours-Proj}} & \multicolumn{4}{c}{\text{Ours}} & \multicolumn{1}{c}{\text{Ours-wo-Bay}}                                                                                                                              \\ \cline{3-11}
                                             &                         & \multicolumn{1}{c}{RE}              & \multicolumn{1}{c}{CD}               & \multicolumn{1}{c}{RC}          & \multicolumn{1}{c}{RE}                 & \multicolumn{1}{c}{CD} & \multicolumn{1}{c}{RC} & \multicolumn{1}{c}{RE} & \multicolumn{1}{c}{CD} & \multicolumn{1}{c}{RC} \\ \midrule[0.03cm]

    \multirow{10}{*}{\textit{SemanticKITTI}} & $00$                    & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \cline{2-11}
                                             & $01$                    & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \cline{2-11}
                                             & $02$                    & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \cline{2-11}
                                             & $03$                    & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \cline{2-11}
                                             & $04$                    & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \cline{2-11}
                                             & $05$                    & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \cline{2-11}
                                             & $06$                    & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \cline{2-11}
                                             & $07$                    & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \cline{2-11}
                                             & $08$                    & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \cline{2-11}
                                             & $09$                    & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \cline{2-11}
                                             & $10$                    & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \hline

    \multirow{4}{*}{\textit{SemanticUSL}}    & $03$                    & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \cline{2-11}
                                             & $12$                    & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \cline{2-11}
                                             & $21$                    & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \cline{2-11}
                                             & $32$                    & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \hline

    \multirow{4}{*}{\textit{FusionPortable}} & \textit{canteen\_day}   & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \cline{2-11}
                                             & \textit{canteen\_night} & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \cline{2-11}
                                             & \textit{garden\_day}    & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \cline{2-11}
                                             & \textit{garden\_night}  & \multicolumn{1}{c}{0}               & \multicolumn{1}{c}{0}                & 0                               & \multicolumn{1}{c}{0}                  & \multicolumn{1}{c}{0}  & 0                      & \multicolumn{1}{c}{0}  & \multicolumn{1}{c}{0}  & 0                      \\ \bottomrule
  \end{tabular}
  \label{tab:mapping_result_public_dataset}
\end{table*}

\end{comment}

==> chapter/exp_table_mapping_result_format_2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}

% FusionPortable
% 00 Carteen
% 01 Garden00
% 02 Garden01
% 03 Escalator
% 04 Building

\begin{table*}[t]
  \centering
  \caption{Mapping Results}
  \renewcommand\arraystretch{1.2}
  \renewcommand\tabcolsep{2pt}
  \scriptsize
  % \footnotesize
  % \tiny
  \begin{tabular}{cc|ccccccccccc|cccc|ccccc}
    \Xhline{0.03cm}
    \multirow{2}{*}{Metrics}                                                     &
    \multirow{2}{*}{Methods}                                                     &
    \multicolumn{11}{c|}{\textit{SemanticKITTI} ($\nu=0.25, 0.3\ (00, 02, 08)$)} &
    \multicolumn{4}{c|}{\textit{SemanticUSL} ($\nu=0.25$)}                       &
    \multicolumn{5}{c}{\textit{FusionPortable} ($\nu=0.25$)}                                                                                                                                                                                                                           \\ \cline{3-22}
                                                                                 &
                                                                                 &
    \rotatebox{0}{00}                                                            &
    \rotatebox{0}{01}                                                            &
    \rotatebox{0}{02}                                                            &
    \rotatebox{0}{03}                                                            &
    \rotatebox{0}{04}                                                            &
    \rotatebox{0}{05}                                                            &
    \rotatebox{0}{06}                                                            &
    \rotatebox{0}{07}                                                            &
    \rotatebox{0}{08}                                                            &
    \rotatebox{0}{09}                                                            &
    \rotatebox{0}{10}                                                            &
    \rotatebox{0}{03}                                                            &
    \rotatebox{0}{12}                                                            &
    \rotatebox{0}{21}                                                            &
    \rotatebox{0}{32}                                                            &
    \rotatebox{0}{00}                                                            &
    \rotatebox{0}{01}                                                            &
    \rotatebox{0}{02}                                                            &
    \rotatebox{0}{03}                                                            &
    \rotatebox{0}{04}                                                                                                                                                                                                                                                                  \\ \Xhline{0.03cm}
    \multirow{3}{*}{RE $[cm]\downarrow$}                                         &
    VoxField                                                                     &
    $7.9$                                                                        & 
    $7.9$       & 
    $7.0$       & 
    $6.6$       & 
    $7.6$       & 
    $7.2$       & 
    $7.1$       & 
    $7.2$       & 
    $\bm{7.9}$  & 
    $6.6$       & 
    $6.6$       & 
    $7.5$       & 
    $7.2$       & 
    $8.2$       & 
    $7.9$       &
    $9.9$       & 
    $13.5$      & 
    $15.2$      & 
    $10.3$      & $15.2$                                                                                                                                                    \\
                                                                                 &
    Ours-Proj                                                                    &
    $7.8$                                                                        & 
    $7.3$       & 
    $6.8$       & 
    $6.3$       & 
    $7.0$       & 
    $6.9$       & 
    $7.0$       & 
    $6.8$       & 
    $8.4$       & 
    $6.2$       & 
    $6.1$       & 
    $7.2$       & 
    $7.4$       & 
    $7.1$       & 
    $7.0$       &
    $9.1$       & 
    $13.4$      & 
    $15.5$      & 
    $9.5$       & $14.2$                                                                                                                                                    \\
                                                                                 &
    Ours                                                                         &
    $\bm{7.5}$                                                                   & 
    $\bm{7.5}$  & 
    $\bm{6.4}$  & 
    $\bm{5.9}$  & 
    $\bm{6.9}$  & 
    $\bm{6.6}$  & 
    $\bm{6.7}$  & 
    $\bm{6.5}$  & 
    $8.1$       & 
    $\bm{5.8}$  & 
    $\bm{5.8}$  & 
    $\bm{6.8}$  & 
    $\bm{7.0}$  & 
    $\bm{6.7}$  & 
    $\bm{6.7}$  &
    $\bm{8.7}$  & 
    $\bm{12.7}$ & 
    $\bm{14.9}$ & 
    $\bm{8.9}$  & 
    $\bm{13.8}$                                                                                                                                               \\ \Xhline{0.01cm}
    \multirow{3}{*}{CD $[cm]\downarrow$}                                         &
    VoxField                                                                     &
    $6.2$                                                                        & 
    $\bm{7.5}$  & 
    $7.1$       & 
    $5.1$       & 
    $\bm{12.7}$ & 
    $5.6$       & 
    $4.7$       & 
    $5.2$       & 
    $8.9$       & 
    $5.1$       & 
    $4.7$       & 
    $\bm{6.3}$  & 
    $\bm{8.7}$  & 
    $\bm{9.6}$  & 
    $\bm{10.8}$ &
    $11.5$      & 
    $13.8$      & 
    $11.9$      & 
    $12.1$      & $12.0$                                                                                                                                                    \\
                                                                                 &
    Ours-Proj                                                                    &
    $6.3$                                                                        & 
    $10.0$      & 
    $7.6$       & 
    $5.2$       & 
    $13.0$      & 
    $5.4$       & 
    $4.9$       & 
    $5.4$       & 
    $7.6$       & 
    $5.1$       & 
    $4.8$       & 
    $6.9$       & 
    $9.0$       & 
    $10.1$      & 
    $11.5$      &
    $9.1$       & 
    $13.3$      & 
    $12.2$      & 
    $10.0$      & $11.2$                                                                                                                                                    \\
                                                                                 &
    Ours                                                                         &
    $\bm{5.8}$                                                                   & 
    $9.8$       & 
    $\bm{6.5}$  & 
    $\bm{5.0}$  & 
    $12.9$      & 
    $\bm{5.1}$  & 
    $\bm{4.5}$  & 
    $\bm{5.1}$  & 
    $\bm{7.1}$  & 
    $\bm{4.7}$  & 
    $\bm{4.6}$  & 
    $6.8$       & 
    $8.8$       & 
    $9.8$       & 
    $11.5$      &
    $\bm{8.2}$  & 
    $\bm{12.7}$ & 
    $\bm{11.0}$ & 
    $\bm{9.2}$  & $\bm{10.5}$                                                                                                                                               \\ \Xhline{0.01cm}
    \multirow{3}{*}{RC $[\%]\uparrow$}                                           &
    VoxField                                                                     &
    $\bm{94.2}$                                                                  & 
    $\bm{87.7}$ & 
    $92.8$      & 
    $\bm{95.7}$ & 
    $\bm{64.1}$ & 
    $93.4$      & 
    $95.8$      & 
    $\bm{95.5}$ & 
    $84.7$      & 
    $\bm{95.9}$ & 
    $\bm{96.5}$ & 
    $\bm{91.5}$ & 
    $\bm{83.6}$ & 
    $\bm{81.9}$ & 
    $\bm{78.2}$ &
    $69.5$      & 
    $63.3$      & 
    $75.3$      & 
    $67.7$      & $80.9$                                                                                                                                                    \\
                                                                                 &
    Ours-Proj                                                                    &
    $93.4$                                                                       & 
    $75.3$      & 
    $90.7$      & 
    $94.6$      & 
    $61.8$      & 
    $93.4$      & 
    $95.0$      & 
    $94.1$      & 
    $90.2$      & 
    $94.9$      & 
    $95.1$      & 
    $88.6$      & 
    $81.8$      & 
    $78.4$      & 
    $73.4$      &
    $78.3$      & 
    $64.7$      & 
    $75.3$      & 
    $75.3$      & $83.1$                                                                                                                                                    \\
                                                                                 &
    Ours                                                                         &
    $\bm{94.2}$                                                                  & 
    $75.4$      & 
    $\bm{93.6}$ & 
    $94.7$      & 
    $61.7$      & 
    $\bm{93.7}$ & 
    $\bm{95.9}$ & 
    $94.3$      & 
    $\bm{91.3}$ & 
    $95.4$      & 
    $95.3$      & 
    $88.6$      & 
    $81.8$      & 
    $79.3$      & 
    $73.0$      &
    $\bm{80.7}$ & 
    $\bm{65.3}$ & 
    $\bm{76.7}$ & 
    $\bm{77.1}$ & $\bm{84.0}$                                                                                                                                               \\ \Xhline{0.01cm}
    \multirow{2}{*}{mIoU $[\%]\downarrow$}                                       &
    Ours-wo-Bay                                                                  &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    \textendash                                                                  &
    \textendash                                                                  &
    \textendash                                                                  &
    \textendash                                                                  &
    \textendash                                                                                                                                                                                                                                                                        \\
                                                                                 &
    Ours                                                                         &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    \textendash                                                                  &
    \textendash                                                                  &
    \textendash                                                                  &
    \textendash                                                                  &
    \textendash                                                                                                                                                                                                                                                                        \\ \Xhline{0.01cm}
    \multirow{2}{*}{Acc $[\%]\uparrow$}                                          &
    Ours-wo-Bay                                                                  &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    \textendash                                                                  &
    \textendash                                                                  &
    \textendash                                                                  &
    \textendash                                                                  &
    \textendash                                                                                                                                                                                                                                                                        \\
                                                                                 &
    Ours                                                                         &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    $0$                                                                          &
    \textendash                                                                  &
    \textendash                                                                  &
    \textendash                                                                  &
    \textendash                                                                  &
    \textendash                                                                                                                                                                                                                                                                        \\
    \Xhline{0.01cm}

    \multirow{2}{*}{Time $[ms]\downarrow$}                                       &
    VoxField                                                                     &
    $109.2$                                                                      &
    $145.0$                                                                      &
    $114.4$                                                                      &
    $132.2$                                                                      &
    $148.3$                                                                      &
    $126.4$                                                                      &
    $151.9$                                                                      &
    $113.8$                                                                      &
    $119.5$                                                                      &
    $135.4$                                                                      &
    $114.8$                                                                      &
    $190.5$                                                                      &
    $210.0$                                                                      &
    $162.2$                                                                      &
    $158.2$                                                                      &
    $326.1$                                                                      &
    $277.7$                                                                      &
    $319.1$                                                                      &
    $161.9$                                                                      &
    $279.1$                                                                                                                                                                                                                                                                            \\
                                                                                 &
    Ours                                                                         &
    $\bm{2.2}$                                                                   &
    $\bm{3.8}$                                                                   &
    $\bm{2.3}$                                                                   &
    $\bm{2.9}$                                                                   &
    $\bm{3.4}$                                                                   &
    $\bm{2.4}$                                                                   &
    $\bm{3.4}$                                                                   &
    $\bm{2.3}$                                                                   &
    $\bm{2.7}$                                                                   &
    $\bm{2.9}$                                                                   &
    $\bm{2.2}$                                                                   &
    $\bm{4.4}$                                                                   &
    $\bm{5.9}$                                                                   &
    $\bm{5.3}$                                                                   &
    $\bm{4.9}$                                                                   &
    $\bm{1.6}$                                                                   &
    $\bm{1.9}$                                                                   &
    $\bm{1.8}$                                                                   &
    $\bm{1.5}$                                                                   &
    $\bm{2.1}$                                                                                                                                                                                                                                                                         \\
    \Xhline{0.03cm}
  \end{tabular}
  \label{tab:mapping_result_public_dataset}
\end{table*}



==> chapter/related_work_navigation.tex <==
\subsection{Geometry and Semantics-Driven Navigation}

Heiden et al. \cite{heiden2018gradient} proposed xxx


==> chapter/related_work_semanticmapping.tex <==
\subsection{Semantic Mapping}

Herb et al. \cite{herb2021lightweight} proposed a semantic mapping framework directly on meshes.

Gan et al. \cite{gan2020bayesian} xxx.
This work \cite{gan2022multitask} focuses on applying the proposed mapping framework
to build a second traversability layer on top of the first
semantic layer developed in the authors' previous work \cite{gan2020bayesian}

Tian et al. (Kimera-Multi)


==> chapter/related_work_teachandrepeat.tex <==



\subsection{Volumetric Mapping}



Herb et al. \cite{herb2021lightweight} proposed a semantic mapping framework directly on meshes.

Gan et al. \cite{gan2020bayesian} xxx.
This work \cite{gan2022multitask} focuses on applying the proposed mapping framework
to build a second traversability layer on top of the first
semantic layer developed in the authors' previous work \cite{gan2020bayesian}

Tian et al. (Kimera-Multi)


\subsection{Navigation in Unstructured Environments}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Teach and Repeat}
\subsubsection{LiDAR-based Teach and Repeat}

(a) Sprunk et al. \cite{sprunk2013lidar} proposed a lidar-based teach-and-repeat system, where laser scans are used to localize the ground vehicle against its taught path driven by the user.

(b) Furgale et al. \cite{furgale2014there,krusi2015lighting} (for repeating long-term motions in highly dynamic environments). Local planner: sample local trajectory to avoid dynamic elements. Map maintenance: identify moving objects and estimate objects' velocities.

\subsubsection{Visual Teach and Repeat}
%%%%% 
Defined in VT and R3\footnote{\url{https://utiasasrl.github.io/vtr3}}\footnote{\url{https://github.com/utiasASRL/vtr3/wiki/Introduction-to-VTR3}}:
Visual Teach and Repeat (VT\&R) is a navigation system for mobile robots.
In the \textbf{teach} phase, a user drives the robot manually to teach a path, while the system builds a map.
Afterward, during the \textbf{repeat} phase, the map is used for localization as the robot follows the path autonomously.
VT\&R relies on local submaps only, which facilitates repetition of long paths without the need for accurate global reconstruction.

%%%%% 
(a) Furgale et al. \cite{furgale2010visual} advanced the local route following in the repeat phase without keeping the global consistency based on the submap.
\textbf{Route teach}:
involves driving the path once while logging stereo images and then postprocessing the image sequence into a series of overlapping submaps.
\textbf{Route repeat}:
robot uses the database of submaps to repeat the route. The system we have implemented can start at any place along the path and repeat the route in either direction, provided that the camera is facing the same direction it was facing during the teach pass

%%%%% 
(b) Paton et al. \cite{paton2018expanding} proposes a multi-experience localization algorithm based on the topometric pose graph presented in \cite{furgale2010visual}.

(c) Light and terrain changes are included in \cite{paton2015s,berczi2016s}, for further improving the accuracy and robustness of state estimation.

(d) Authors in \cite{ostafew2013visual} developed an iterative learning controller (ILC) to reduce the tracking error when the robot executes the teaching path.

\subsubsection{Teach and Repeat with a UAV}
%%%%% 
(a) Quadrotor teach and repeat work presented in \cite{fehr2018visual} uses a vision-based drone to conduct a repetitive inspection by demonstrating the desired path and selecting some checkpoints.

(b) Gao et al. \cite{gao2019optimal}, \textbf{Teach}: build the map of the surrounding environment and convert the recorded trajectory into a topological trajectory;
\textbf{Repeat}, the planning framework optimizes the trajectory in both spatial (free space) and temporal (minimum-time temporal trajectory) aspects. But weaknesses: environment remains intact; perfect localization; axis-aligned cubes not good to cover large free space.

(c) Gao et al. \cite{gao2020teach} extended its work, by adapting to arbitrarily cluttered maps and providing sufficient solution space. \textbf{Before teaching}: build the global map. \textbf{Teach}: generate the topological map and flight corridor; optimize spatial and temporal trajectories and local planner to run to avoid obstacles.
\textbf{Repeat}: generate local ESDF map and local planning and replanning.
Compared with \cite{furgale2010visual,paton2018expanding,ostafew2013visual,fehr2018visual}, key features of Gao's works:
\begin{itemize}
    \item More smooth trajectory: converts an arbitrarily poor path to a safe and efficient trajectory with expected flying aggressiveness.
    \item Flexible, no need for manual control: since it records the teaching path by virtually controlling the drone in simulation, a manually piloted teaching process is unnecessary.
    \item Robust: to environmental changes and can even avoid moving obstacles.
    \item Globally consistent localization and mapping.
\end{itemize}

%%%%%%%%%%%%%%%%
\subsubsection{Our work}
The key differences/improvements compared with existing works are
\begin{itemize}
    \item We propose a complete method to build the large-scale metric-semantic map in real-time, including the state estimation, perception, and mapping. The new metric-semantic map can provide lots of information: reversibility, traffic rule, terrain assessment through the vision, etc.
    \item Flexible: no need for serious manual driving trajectory. Any trajectories will be generated from any start and goal point.
    \item Globally consistent localization and mapping.
\end{itemize}

